Search for pairs of highly collimated photon-jets in $pp$ collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector

Results of a search for the pair production of photon-jets$-$collimated groupings of photons$-$in the ATLAS detector at the Large Hadron Collider are reported. Highly collimated photon-jets can arise from the decay of new, highly boosted particles that can decay to multiple photons collimated enough to be identified in the electromagnetic calorimeter as a single, photonlike energy cluster. Data from proton-proton collisions at a center-of-mass energy of 13 TeV, corresponding to an integrated luminosity of 36.7 fb$^{-1}$, were collected in 2015 and 2016. Candidate photon-jet pair production events are selected from those containing two reconstructed photons using a set of identification criteria much less stringent than that typically used for the selection of photons, with additional criteria applied to provide improved sensitivity to photon-jets. Narrow excesses in the reconstructed diphoton mass spectra are searched for. The observed mass spectra are consistent with the Standard Model background expectation. The results are interpreted in the context of a model containing a new, high-mass scalar particle with narrow width, $X$, that decays into pairs of photon-jets via new, light particles, $a$. Upper limits are placed on the cross section times the product of branching ratios $\sigma \times \mathcal{B}(X \rightarrow aa) \times \mathcal {B}(a \rightarrow \gamma \gamma)^{2}$ for 200 GeV $< m_{X} <$ 2 TeV and for ranges of $ m_a $ from a lower mass of 100 MeV up to between 2 and 10 GeV, depending upon $ m_X $. Upper limits are also placed on $\sigma \times \mathcal{B}(X \rightarrow aa) \times \mathcal {B}(a \rightarrow 3\pi^{0})^{2}$ for the same range of $ m_X $ and for ranges of $ m_a $ from a lower mass of 500 MeV up to between 2 and 10 GeV.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 14-Feb-2018

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DRF/IRFU, France; SRNSFG, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, the Canada Council, CANARIE, CRC, Compute Canada, FQRNT, and the Ontario Innovation Trust, Canada; EPLANET, ERC, ERDF, FP7, Horizon 2020 and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d'Avenir Labex and Idex, ANR, R{\'e}gion Auvergne and Fondation Partager le Savoir, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF; BSF, GIF and Minerva, Israel; BRF, Norway; CERCA Programme Generalitat de Catalunya, Generalitat Valenciana, Spain; the Royal Society and Leverhulme Trust, United Kingdom.

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------



==> EXOT-2017-08-metadata.tex <==
\AtlasJournalRef{Phys. Rev. D 99, 012008}
\AtlasDOI{10.1103/PhysRevD.99.012008}

\AtlasTitle{
	Search for pairs of highly collimated photon-jets in $pp$ collisions at $\sqrt{s}$ = 13~\TeV\ with the ATLAS detector
}

%\AtlasVersion{3.4}

\AtlasRefCode{EXOT-2017-08}

\AtlasJournal{PRD}

\AtlasAbstract{%
Results of a search for the pair production of photon-jets---collimated groupings of photons---in the ATLAS detector at the Large Hadron Collider are reported.
Highly collimated photon-jets can arise from the decay of new, highly boosted particles that can decay to multiple photons collimated enough to be identified in the electromagnetic calorimeter as a single, photon-like energy cluster.
Data from proton--proton collisions at a center-of-mass energy of 13~\TeV, corresponding to an integrated luminosity of 36.7~fb$^{-1}$, were collected in 2015 and 2016.
Candidate photon-jet pair production events are selected from those containing two reconstructed photons using a set of identification criteria much less stringent than that typically used for the selection of photons, with additional criteria applied to provide improved sensitivity to photon-jets.
Narrow excesses in the reconstructed diphoton mass spectra are searched for.
The observed mass spectra are consistent with the Standard Model background expectation.
The results are interpreted in the context of a model containing a new, high-mass scalar particle with narrow width, $X$, that decays into pairs of photon-jets via new, light particles, $a$.
Upper limits are placed on the cross-section times the product of branching ratios $\sigma \times {\mathcal {B}}(X \rightarrow aa) \times {\mathcal {B}}(a \rightarrow \gamma \gamma)^{2}$ for $200~\GeV< m_{X} <2~\TeV$ and for ranges of $ m_a $ from a lower mass of $ 100~\MeV $ up to between $ 2~\GeV $ and $ 10~\GeV $, depending upon $ m_X $.
Upper limits are also placed on $\sigma \times {\mathcal {B}}(X \rightarrow aa) \times {\mathcal {B}}(a \rightarrow 3\pi^{0})^{2}$ for the same range of $ m_X $ and for ranges of $ m_a $ from a lower mass of $ 500~\MeV $ up to between $ 2~\GeV $ and $ 10~\GeV $.
}

\PreprintIdNumber{CERN-EP-2018-143}

